Serving the Grid: an Experimental Study of Server Clusters as Real-Time Demand Response Resources

Demand response is a crucial technology to allow large-scale penetration of intermittent renewable energy sources in the electric grid. This paper is based on the thesis that datacenters represent especially attractive candidates for providing flexible, real-time demand response services to the grid; they are capable of finely-controllable power consumption, fast power ramp-rates, and large dynamic range. This paper makes two main contributions: (a) it provides detailed experimental evidence justifying this thesis, and (b) it presents a comparative investigation of three candidate software interfaces for power control within the servers. All of these results are based on a series of experiments involving real-time power measurements on a lab-scale server cluster. This cluster was specially instrumented for accurate and fast power measurements on a time-scale of 100 ms or less. Our results provide preliminary evidence for the feasibility of large scale demand response using datacenters, and motivates future work on exploiting this capability.

==> methods.tex <==
\FloatBarrier
\section{Methods}\label{sec:methods}

\begin{sidewaysfigure*}
	\centering
	\includegraphics[width=\textwidth]{measuredPowerConsumption}
	\caption{Test text}
	\label{fig:measuredPowerConsumption}
\end{sidewaysfigure*}

\subsection{Experimental setup}
The experimental setup is a Dell PowerEdge R320 server with an Intel Xeon E5-2400 series processor, running Ubuntu 12.04 with the 3.16.0-41-generic Linux kernel. We've instrumented the server with a current sensor for validation of the on-chip power usage estimate obtained through the software interface. During each test, the Linux stress program \cite{stressProgram} (running repeated square root operations) was used as the workload, with the exception of \cref{fig:stress}, which used a simplified version of the stress program, modified to include custom delays. Each test ran for 15 seconds of data at each control setpoint, and ran each control setpoint twice for comparison. The package power was estimated using the RAPL interface, and was sampled once ever 150 milliseconds.

\subsection{Results}
At full load, the server consumes about 85 W. At idle, the server consumes around 55 W. This means that 30\% of the capacity of the IT load is accessible to demand response. For example, in a 50 MW datacenter like [cite], running at a PUE of 1.5, the IT load capacity is 33.3 MW, which assuming that each computer had same dynamic range as our PowerEdge R320, would correspond to 10 MW of demand response potential -- an order of magnitude greater than the 1 MW minimum deferrable load requirement [cite] to qualify as a controllable load resource.

The plots below are a standard box plot, with the box representing the interquartile range (IQR) for the power at each control input value and the whiskers representing the minimum and maximum values. The outliers (greater than 10 times IQR) are shown in red.

\subsubsection{Direct DVFS}

The acpi-cpufreq driver is the predecessor to the more recent intel\_pstate driver used in modern servers. Unlike the more recent driver, which in the default configuration offloads the majority of power management to the processor itself, the acpi-cpufreq driver uses software to suggest different voltage-frequency pairs called power states (P-states) through the ACPI interface. As mentioned earlier, Intel documentation states that these requests may be overruled by the internal thermal management logic of the processor. However, it has been the experience of the authors that the requested P-state is usually entered unless it is thermally unsafe to do so.

The acpi-cpufreq driver provides of power management policies that the operating system uses to determine which P-state to request and when to do so. The userspace governor allows the user to specify a target frequency, and the driver will determine the corresponding P-state to request. The benefits and drawbacks of this method are shown in \cref{fig:cpufreq}. The main advantage is that the variance of the power is very low (notice how tight the box plot is). The downsides of this technique are two. First, the range of power levels is relatively small -- starting at 24 watts, over twice the idle power consumption. This is due to the operating system never placing the processor in a sleep state. Second, the number of unique power levels available is quite small (only twelve on the processor used in this study). This is due to the processor having a limited number of P-states available for DVFS.

\subsection{Proprietary On-chip Power-Limiting}

Intel published results from an early version of RAPL in 2010 which was capable of finely shaping the power consumption of memory by rapidly switching between adjacent memory bandwidth states \cite{RAPL}. While, the current implentation which is capable of shaping the power consumption of both memory and processor package is proprietary, the limiting value around 24 W suggests that a similar technique using P-states is used for shaping processor power. It is also fairly evident that the RAPL interface for the processor used in this study does not transition the processor to sleep states.

This technique has the advantage of providing very tight control over a wide range of power values between around 24 watts and the maximum power. The primary disadvantage, as \cref{fig:rapl} shows, is that similar to the cpufreq method, RAPL does not allow power to be capped across the full range of server power consumptions. Moreover, because not all processors (even within the Intel Xeon family) support RAPL power limiting features, the technique may not be an option for many server configurations.

\subsubsection{Hypervisor CPU capping}

The Xen Project hypervisor \cite{BarhamXen2003} is a type-1 (also called ``baremetal'') hypervisor, which means that it runs architecturally ``beneath'' any guest operating systems that it is coordinating. While VMWare remains the industry defacto standard, Xen has a wide deployment (in 2012, it held the second-largest market share of any virtualization technology \cite{aberdeen2012}) and has the advantage of being free and open source software. Xen contains a variety of resource contention management features, including a processor utilization capping mechanism called sched-credit. The current implementation uses a priority queue and an accounting thread to ensure that the virtual CPUs assigned to the virtual machines do not exceed their CPU utilization cap.

\cref{fig:hypervisor} are results gathered cpu capping a paravirtualized linux guest VM allocated four virtual CPUs and running four threads of the stress program. One advantage of this technique is that it offers a full range of power values between idle maximum power. The reason it is able to achieve low power values is that hypervisor is allowed to transition the processor to a sleep state for a portion of each 30 ms accounting period (when the guest VM has exceeded its allotted allocation credits).

The primary downside of this technique is that it is difficult to tightly control the power consumption at power levels corresponding to hypervisor allocation settings which cause the number of physical cores allocated to the guest operating system to oscillate. Note, for example, the increased variance at 200 allocation points -- where the guest operating system is alternately being allocated between two and three physical cores. Similarly, there is another jump in power variance at 300 allocation points.

\subsection{Intel PowerClamp}
The Intel PowerClamp driver was developed to force the processor to enter certain sleep states through synchronized idle injection across all threads \cite{powerclamp}. The driver implements a closed loop control with limits on the amount of idle time that can be injected.

While the system is indeed entering sleep states during the lower-power portions of \cref{fig:powerclamp}, the fact that idle injection is limited to 50\% idle time means that the power of the fully-loaded system still cannot be reduced below about 17 W. Moreover, compared to the hypervisor solution, there is a relatively large spread in power at every control setpoint.

\subsection{Power-aware Workload}

The authors have provided two custom software solutions for comparison with the aforementioned power-shaping technologies. The first of these is a baseline ``best-case scenario'' workload which has been specifically tailored to use a certain percentage of each processor. Each of the four threads in the workload uses POSIX timers and the usleep() command to insert delays between blocks of 50000 square root operations. The amount of delay was calculated to correspond to a specified CPU utilization. An ad hoc procedure was used to tune the number of square root operations and the number of threads to achieve the maximum dynamic range of power.

The benefit of such a workload is clear. Not only is there a roughly linear correspondence between CPU utilization and power consumption, but the variance at each setpoint is relatively small, and the full dynamic range of power consumption is achievable. The downside of this technique is that it is extremely invasive -- requiring a rewrite of all CPU-intensive software on the system.

\subsection{Custom Userspace Software}
\cref{fig:insertDelays}
To provide a comparison and a more general method for inserting delays in the user space, the authors designed a tool which modulates the CPU utilization of processes using the Linux SIGSTOP and SIGCONT signals in a manner inspired by the cpulimit \cite{cpulimit} program. Because this program is running in userspace, it was expected to have significantly increased power variance compared to the powerclamp driver. However, while the worst-case power bounds did indeed increase, the variance was comparable to that afforded by the powerclamp driver.

The advantage of such a tool is that it can be run in the background of any POSIX operating system, without the need for accessing custom MSRs, modifying hypervisor power management policies, or kernel drivers. The disadvantage is that the variance is larger than some of the other methods.
